Efficient Race Detection with Futures

This paper addresses the problem of provably efficient and practically good on-the-fly determinacy race detection in task parallel programs that use futures. Prior works determinacy race detection have mostly focused on either task parallel programs that follow a series-parallel dependence structure or ones with unrestricted use of futures that generate arbitrary dependences. In this work, we consider a restricted use of futures and show that it can be race detected more efficiently than general use of futures. Specifically, we present two algorithms: MultiBags and MultiBags+. MultiBags targets programs that use futures in a restricted fashion and runs in time $O(T_1 \alpha(m,n))$, where $T_1$ is the sequential running time of the program, $\alpha$ is the inverse Ackermann's function, $m$ is the total number of memory accesses, $n$ is the dynamic count of places at which parallelism is created. Since $\alpha$ is a very slowly growing function (upper bounded by $4$ for all practical purposes), it can be treated as a close-to-constant overhead. MultiBags+ an extension of MultiBags that target programs with general use of futures. It runs in time $O((T_1+k^2)\alpha(m,n))$ where $T_1$, $\alpha$, $m$ and $n$ are defined as before, and $k$ is the number of future operations in the computation. We implemented both algorithms and empirically demonstrate their efficiency.

==> Makefile <==
# Standard Makefile for compiling LaTeX documents in the Supertech
# group.

DOC=main

# This line is intentionally blank.

TARGETS=$(patsubst %,%.pdf,$(DOC))

OTHERS = Makefile # plain-url.bst supertech.sty allpapers.bib

DEPS_DIR = .deps

INCLUDE_DIR=.

LATEXMK = TEXINPUTS=$(INCLUDE_DIR)/: BIBINPUTS=$(INCLUDE_DIR)/: BSTINPUTS=$(INCLUDE_DIR)/: latexmk
LATEXMK_FLAGS = -pdflatex="pdflatex --shell-escape %O %S" -pdf -dvi- -ps- -recorder -M -MP \
                  -e 'show_cus_dep();' \

default: pdf
.PHONY:  pdf default all remake clean allclean

all: $(TARGETS)

-include $(DEPS_DIR)/$(DOC).pdfP

ifneq (,$(findstring B,$(MAKEFLAGS)))
LATEXMK_FLAGS += -gg
endif

$(DEPS_DIR) :
	if [ ! -d $(DEPS_DIR) ]; then mkdir $@; fi

$(DOC).pdf : $(OTHERS)

###########################################################################
## Make targets for cleaning

clean%:
	rm -f $*.aux $*.ps $*.pdf $*.dvi $*.bbl $*.blg $*.tmp $*.lof $*.log $*.toc $*.out $*.fls $*.fdb_latexmk $(DEPS_DIR)/$*.pdfP *~ *.tex.bak

clean: clean$(DOC)

allclean:
	rm -f *.aux *.dvi *.bbl *.blg *.tmp *.lof *.log *.toc *.out *.fls *.fdb_latexmk $(DEPS_DIR)/*.pdfP $(DOC).pdf *~



###########################################################################
## Make targets for document

pdf : $(DOC).pdf

%.pdf : %.tex $(OTHERS)
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) $(LATEXMK_FLAGS) -MF $(DEPS_DIR)/$@P $<
	if [ -e $@ ]; then touch $@; fi

# Some nonsense that latexmk doesn't understand with minted can be fixed by telling that these rules are easy.
%.w18 %.out.pyg %.aex: %.tex
	@echo > /dev/null
# remake :
# 	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
# 	$(LATEXMK) -g -deps-out=$(DEPS_DIR)/$(DOC).pdfP $(DOC).tex
# 	if [ -e $(DOC).pdf ]; then touch $(DOC).pdf; fi


==> concl.tex <==
\secput{concl}{Conclusion}

This paper provides a race-detection algorithm for unstructured
futures that runs in $O(T_1 + k^2)$ time, with an additive overhead
quadratic in the number of \getF operations.  Note that if one is not
careful, a program with unstructured futures can deadlock.  Such a
deadlock is deterministic, however, and does not depend on the
schedule.  In such cases, our algorithm race detects until the
execution deadlocks.  When the use of futures is structured, we
provide a race detection algorithm with almost no asymptotic overhead.

Currently, both of our algorithms execute the computation serially.
An interesting avenue of future work is how to parallelize these.
Both our algorithms depend on depth-first execution order and
extension to parallel execution appears to be non-trivial.


% Note: restriction --- talk about how unstructured use of future 
% may deadlock 


==> cut/abstract.tex <==
\begin{abstract}
  This paper addresses the problem of provably-efficient and
  practically good on-the-fly race detection in programs with futures.
  \defn{Determinacy races} occur in a parallel program when two
  logically parallel instructions access the same memory location and
  at least one of the accesses is a write. These can lead to
  non-deterministic behavior and thus are often difficult-to-find
  bugs. We consider race detection for \defn{dynamically multithreaded
    programs}, where the programmer expresses the logical parallelism
  of the program in a processor-oblivious manner and lets the runtime
  system schedule the program.

  Most prior work on race detection for dynamically multithreaded
  programs is restricted to programs that follow a series-parallel
  dependence structure. This paper presents race-detection algorithms
  for a more general class of programs, namely programs that use
  futures, in addition to series-parallel constructs, to express
  parallelism.

  Specifically, we present two algorithms: \MultiBags and
  \MultiBagsPlus.  \MultiBagsPlus race detects programs that employ
  unrestricted use of futures, and runs in time
  $O((T_1+k^2)\iack(m,n))$ where $T_1$ is the sequential running time
  of the program, $\iack$ is the inverse Ackermann's function, $m$ is
  the total number of memory accesses, $n$ is the dynamic count of
  places at which parallelism is created, and $k$ is the number of
  future operations in the computation.  This running time has an
  additive $k^2$ overhead on top of the sequential running time ---
  $\iack$ can be treated as a close-to-constant overhead since it is a
  slowly growing function (upper bounded by $4$).  Since general use
  of futures can generate arbitrary dependence structures, it seems
  unlikely that one can race detect with no or small overhead. We also
  propose \MultiBags, which targets programs that use futures in a
  restricted fashion. \MultiBags runs in time $O(T_1 \iack(m,n))$. We
  implemented both algorithms and empirically demonstrate their
  efficiency.

  %% Interestingly, we observe that when a program uses futures in 
  %% a restricted fashion, it's possible to detect races more efficiently.
  %% Via this observation, we also propose \MultiBags, which targets programs 
  %% that use futures in a restricted fashion, where the restrictions can be
  %% checked conservatively by a compiler.  \MultiBags runs in time $O(T_1 \iack(m,n))$,
  %% which is $O(T_1)$ for all intents and purposes. 

\end{abstract}

\punt{
  Since $\iack$ is a very slow growing function 
  (upper bounded by $4$), our algorithm is almost asymptotically the same
  as the state-of-the-art algorithm proposed by~\citet{AgrawalDeFi18}, 
  which runs in time $O((T_1+k^2)\iack(m,n))$.  The state-of-the-art
  algorithm, however, is theoretical and cannot be implemented 
  efficiently.  \MultiBagsPlus, on the other hand, can be implemented 
  efficiently in practice, and we demonstrate that empirically.  

  Interestingly, we observe that, programs that use futures in a restricted
  way can be race detected efficiently.  Given this observation, we define
  the restrictions precisely, which can be checked conservatively by a
  compiler, and propose a second algorithm, \MultiBags, that target such 
  restricted use of futures.  \MultiBags runs in time $O(T_1 \iack(m,n))$,
  which is $O(T_1)$ for all intents and purposes. 
}



==> motivation.tex <==
\secput{motivation}{Distinctions between Structured versus General Futures} 

In this section, we discuss the motivations for distinguishing
structured futures versus general futures.  Structured futures
generalize fork-join parallelism --- any program that can be expressed
using fork-join parallelism can be expressed using structured futures.
However, they still impose some restrictions. General futures
essentially enable arbitrary dependencies to be formed among logically
parallel subcomputations, thereby allowing an even larger class of
programs than structured futures. Structured futures can enable higher
parallelism than fork-join constructs alone, and general futures can
further enable more parallelism. Moreover, the use futures make it
easier to express some types of parallelism.

%% However, under the premise that
%% programs that race detection can be performed more efficiently for
%% structured future-parallel programs, we ask the following questions:
%% %utilize only structured futures can be race-detected
%% %more efficiently, 

%% \begin{closeitemize}
%% \item are there useful programs one could write using
%%   structured futures; and
%% \item are general futures useful over structured futures?
%% \end{closeitemize}

%% With simple programming examples, we show that, the structured futures
%% can enable higher parallelism compared to using fork-join constructs
%% alone, and general futures can further enable higher parallelism
%% compared to structured futures.  Moreover, the use of futures make it
%% easier to express some types of parallelism where restricting
%% to fork-join parallelism either significantly reduces
%% parallelism or makes programming much harder. 

%% \subsection*{Motivating example: least common subsequence}

We illustrate the difference between these forms of parallelism using
a the longest common subsequence (LCS) problem.  For simplicity, we
assume that the two input strings have the same length, $N$.  One can
think of the computation of LCS effectively as filling out an
$N$-by-$N$ table.  Given two strings $X$ and $Y$, the cell $(i,j)$
computes the longest common subsequence between the prefix of $X$ up
to the $i^\text{th}$ character and the prefix of $Y$ up to the
$j^\text{th}$ character.
\figref{lcs-dep} shows the dependence structure of LCS:
we compute the value at cell $(i,j)$ by looking at the computed
values at its neighboring cells $(i-1, j)$ (neighbor to its left), 
$(i-1, j-1)$ (neighbor to its upper left), and $(i, j-1)$ 
(neighbor above it).  Note that many dynamic programming examples can 
be computed similarly thus have the same dependence structure.
         
\begin{figure}[t]
\begin{minipage}[c]{0.34\linewidth}
\includegraphics[width=2.5cm]{figures/lcs-dep}
\end{minipage}
\hspace{-3mm}
\begin{minipage}{0.66\linewidth}
\vspace{-4mm}
\caption{LCS data dependencies.  Given input strings $X$ and $Y$,
cell $(i,j)$ computes the longest common subsequence between 
the prefix of $X$ (up to the $i^{th}$ char) and prefix $Y$ 
(up to the $j^{th}$ char).  The red arrows denote the data flow.}
%  The implementation
% with the coarsened base case has the same data dependencies.}
\label{fig:lcs-dep}
\end{minipage}
\end{figure}

\begin{figure}[t]
\begin{minipage}[c]{0.30\linewidth}
\includegraphics[width=2.4cm]{figures/structured-dep}%
\end{minipage}
\hspace{-3mm}
\begin{minipage}{0.70\linewidth}
\vspace{-4mm}
\caption{The dag of LCS using structured futures.
The large circles represent the processing of a block, and the 
small circles represent strands that invoke \createF to process 
a block and \getF to wait for the processing.  Wiggly arrows 
denote non-SP edges due to \createF (solid) and \getF 
(dotted) calls.}%
\label{fig:structured-dag}%
\end{minipage}\\
\end{figure}

\paragraph{Parallelizing LCS with fork-join parallelism:}
To parallelize LCS using fork-join parallelism, one can traverse each
of the diagonal wavefront one after another, but compute the cells
within a single wavefront in parallel using a parallel for loop. Such
parallelization leads to a work of $\Theta(N^2)$ and span of
$\Theta{(N \lg N)}$. In practice, one would normally coarsen the base
case to $B$-by-$B$ cells to reduce the spawning overhead. We then have
$\frac{N}{B}$ wavefronts, leading to a span of $\Theta(BN
+ \frac{N}{B}\lg\frac{N}{B})$

%% The
%% total work of LCS is $\Theta(N^2)$, since there are a total of $N^2$
%% cells, each requires constant work.  Such a parallelization leads to a
%% span of $\Theta{(N \lg N)}$, since processing each wavefront with $k$
%% cells has a span of $\lg k$, and the wavefronts are processed one
%% after another, leading to span of $\sum\nolimits_{i=1}^N \lg i =
%% \Theta(N \lg N)$.

%% Spawning until we recurse down to the base case of one single cell can
%% leads to high spawning overhead, and thus, one would normally coarsen
%% the base case.  Assuming we coarsen the base case to be a block of
%% $B$-by-$B$ cells, we then have $\frac{N}{B}$ wavefronts that need to
%% be processed one after another, and blocks within each wavefront can
%% be processed in parallel.  Such a parallelization strategy has the
%% same amount of work, and leads to a span of
%% $\sum\nolimits_{i=1}^{\frac{N}{B}} {B^2} \lg i = \Theta(BN
%% + \frac{N}{B} \lg
%% \frac{N}{B})$. 

\paragraph{Parallelizing LCS with structured futures:}
Structured futures lead to increased parallelism for this example. We
will still traverse the blocks in a wavefront fashion. However, we
will call \createF to spawn off the computation that process each
block and use future handles to enforce the necessary dependencies.
Specifically, we can traverse the wavefronts and spawning off
processing of blocks in such a way that forms the dependence graph
shown in \figref{structured-dag}.  The small circles represent the
traversal of wavefronts that spawn off each block, and a single large
circle represents the processing of a single $B$-by-$B$ block.

Recall that we must follow two restrictions to use structured futures:
a) the future has to be single-touch, and b) the \createF call and
the \getF call must fall on a path so that there is no race on the
future handle.  To follow these constraints, we can only \getF on one
of the blocks that we depend on.  Thus, right before we spawn off the
processing of a block at $(i,j)$, we will invoke \getF on the block
$(i,j-1)$ (one immediately above the current block).  We also need to
satisfy the dependence on block $(i-1,j)$ (one to the left) somehow.
This is achieved by traversing the wavefront in series --- notice that
the small circles in the same wavefront are visited in series.  That
means, before we visit block $(i,j)$ and spawn off its processing, we
have already visited block $(i+1,j-1)$ which invokes \getF on the
future that processes block $(i,j-1)$, thus satisfying the dependence.
We also need to ensure that block $(i-1,j-1)$ is done, which is
transitively satisfied through calling \getF on block $(i,j-1)$.

The work stays the same as the fork-join case: $\Theta(N^2)$.  The span is,
however, $\Theta(BN + N/B)$, by following the longest path
through the dependence dag shown in \figref{structured-dag} (e.g.,
zigzag through the first row that processes blocks $(0,*)$ and go down
down the last column).  When $B = o(\lg N)$, this span is smaller than
the one we get with fork-join parallelism.

\paragraph{Parallelizing LCS with general futures:} Now let's consider
parallelizing LCS with general futures.  General futures have no
restriction on the number of \getF calls per future; moreover, a
strand that invokes \getF may run in parallel with the strand that
invokes \createF on the same future handle, so long as the \getF comes
after \createF in the serial traversal so that the system does not
deadlock when running on one worker.  Thus, we can spawn off all the
future computations that process each block in parallel, and with a
future task that processes block $(i,j)$, we invoke \getF on the
futures that process block $(i-1,j)$ and block $(i,j-1)$ (and note
that the dependence on processing of block $(i-1,j-1)$ must be
transitively satisfied). The resulting algorithm is asymptotically the
same as structured futures but much simpler.

%% Doing so leads to the same amount of work
%% but the span is $\Theta(BN + \lg \frac{N}{B})$. Since the first term
%% dominates, this is asymptotically the same as structured futures, but
%% much simpler.

%% \begin{figure}[!ht]
%% \centering
%% \begin{footnotesize}
%% \setlength\tabcolsep{2pt}
%% \newcommand{\cheader}[3]{\multicolumn{#1}{#2}{\textit{#3}}}
%% \begin{tabular}{r|c|c|c|c}
%% %\hline
%%     & LCS & SW & BST-merge & MM \\ 
%% \hline
%% \textit{work}       & $\Theta(N^2)$ & $\Theta(N^3)$ & $\Theta(N)$ 
%%                     & $\Theta(N^3)$ \\
%% \textit{fork-join span}    & $\Theta(BN+\frac{N}{B}\lg\frac{N}{B})$
%%                     & $\Theta(BN + \frac{N}{B}\lg\frac{N}{B})$
%%                     & $\Theta(\lg^2{N} + B)$ & $\Theta(BN)$ \\
%% \textit{structured span}   & $\Theta(BN + \frac{N}{B})$
%%                              & $\Theta(BN + \frac{N}{B})$ 
%%                              & $\Theta(\lg^2{N} + B)$ & $\Theta(BN)$ \\ 
%% \textit{general span} & $\Theta(BN + \lg \frac{N}{B})$
%%                              & $\Theta(BN + \frac{N}{B})$ 
%%                              & $\Theta(\lg N + B)$ & $\Theta(BN)$ \\
%% %\hline
%% \end{tabular}
%% \caption{The work and span of different implementations to solve
%% least common subsequence (LCS), Smith-Waterman (SW), binary search tree 
%% merge (BST-merge), and matrix multiplication without temporary storage (MM),  
%% for input size is $N$ and base case $B$.}
%% % including the number of stages per iterations, number of iterations, 
%% % and number of memory accesses.
%% \label{fig:workspan}
%% \end{footnotesize}
%% \end{figure}

%% \figref{workspan} summarizes the work and span for different programs 
%% written using fork-join parallelism, structured futures, and general
%% futures.  For LCS (and SW), as we decrease the block size $B$, the gap 
%% of parallelism between using fork-join constructs and structured futures widens, but structured and unstructured futures
%% have the same span.
%% %  (since for small $B$, the term 
%% % $\frac{N}{B} \lg \frac{N}{B}$ dominates the term $BN$).  
%% % Similarly, as we decrease the block size $B$, the parallelism gap between
%% % the implementation that uses structured futures versus one that uses
%% % general futures also widens.  
%% % Smith-waterman (SW), which has similar
%% % dependence structure exhibits similar trend.
%% For binary tree merge, the only possible implementation using
%% structured futures is effectively invoking \createF in place of \spawn
%% and \getF in place of \sync. Thus, the use of the structured futures
%% does not provide any parallelism advantage.  Interestingly, the use of
%% general futures allows pipelining of the merge with the split
%% operation (which is invoked as a subcomputation of merge) thereby
%% reducing the span by a factor of $\lg N$~\cite{BlellochRe97}.  The
%% pipeline is nonlinear, however, and cannot be implemented using
%% structured futures.  For matrix multiplication, the use of futures
%% leads to slightly different implementations compared to fork-join
%% parallelism, but does not lead to asymptotic improvement in parallelism.
Finally, we note that, \emph{linear} pipeline parallelism is yet another 
commonly supported parallel programming patterns (e.g., 
see~\cite{McCoolRoRe12, LeeLeSc13, LeeLeSc15}), which cannot be 
implemented easily using fork-join constructs such as \spawn and \sync,
but it can be implemented using futures (structured or general).  



==> online.tex <==
\section{Model}

We can model computations that employ \spawn, \sync, \createF, and
\getF as generating a set of series parallel dags which are connected
to each other with \defn{non-SP} edges that connect these dags.  These
non-SP edges are incident on strands that end with \createF and start
with \getF instructions.  In particular, a strand that ends with
\createF has two outgoing edges --- one non-SP edge leading to the
first strand in the function invocation associated with the future
creation, and one SP edge leading to the continuation of the parent
function.  A strand that starts with \getF has two incoming edges ---
one SP edge from the strand that precedes the \getF call in the
current function and one non-SP edge from the last strand of the
function invocation associated with the future handle given as input
to \getF.

We will say that a SP dag $A$ is a create-predecessor of SP dag $B$ if
some node in $A$ is connected to the first node in $B$ through
\createF edges.  Similarly, $A$ is a join-successor of $B$ if the last
strand of $B$ is connected to some node in $A$ via join edges.  $A$
can be both a create-predecessor and a join successor of $B$.  In a
create predecessor $A$ of $B$, $u$ is the creator node of $B$ if the
\createF edge for $B$ or some create ancestor of $B$ was incident on
$u$.  We overload notation and say that $u$ is the creator of all
nodes in $B$.  


However, in order to avoid cycles, create predecessor edges form an
out-tree tree between SP dags; similarly join successor edges form an
in-tree between the SP dags.  Therefore between any two SP dags, we
can define a least common create-predecessor and a least common
join-successor.  We will overload notation and say that a dag $A$ is a
least common create predecessor of two nodes $u$ and $v$ if $A$ is the
least common create predecessor of the SP dags containing $u$ and $v$
respectively.  


We have an additional restriction on the computation --- if we execute
the program in the left to right sequential execution order (spawned
functions and created futures always execute before the continuation)
then no strand has to wait on a \getF edge.  

This restriction leads to the following restrictions on the dag.  If
there is a path from a node $u$ to node $v$ via non SP edges including
a \getF edge, then we can look at the least common create ancestor of
$u$ and $v$.  

This leads to some 
restrictions on the dag: If there is a path from a node $u$ to node $v$
in the same series parallel dag through non-SP edges, then $u$
executes before $v$ in the left-to-right sequential order.  If $u$ and
$v$ are in different dags, then there are two cases.  Either $u$ is in
an create-predecessor of $v$ or $v$ is in a join-successor of $u$.
If neither of these is true, then we can look at the least common
create predecessor of $u$ and $v$ and the create predecessor $w$ of
$u$ executes before the create predecessor $x$.  



==> unstruct-construct-code.tex <==
\begin{figure}
\scriptsize
  \begin{tabular}{|l|l|}
  \hline
  \begin{minipage}[t]{0.48\linewidth}
  $u$ is the first strand of the computation:\vspace{-1ex}
  \begin{codebox}
    \li add $u$ to an attached set with no predecessor.  
  \end{codebox}%
  \vspace{-2ex}
\noindent\rule{\linewidth}{0.4pt}
  Function $F$ calls \spawn($G$):\vspace{-1ex}
  \begin{codebox*}
    \zi \RComment $u$ is the strand in $F$ immediately before the \spawn
    \zi \RComment $v$ is the strand in $F$ right after \spawn 
    \zi \RComment $w$ is the first strand of $G$
    \li $S_G \gets \MakeSet(\dssp, w)$ \lilabel{dsspspawn}
    \li $U_v \gets \MakeSet(\dsnsp, v)$ and make $U_v$ unattached.
    \li $\attpred{U_v} \gets \attpred{\find{\dsnsp, u}}$ \lilabel{setAttPredSpawn}
    \li $U_w \gets \MakeSet(\dsnsp, w)$ and make $U_w$ unattached.
    \li $\attpred{U_w} \gets \attpred{\find{\dsnsp, u}}$ \lilabel{setAttPredCont}
  \end{codebox*}
  \vspace{-.5ex}
\noindent\rule{\linewidth}{0.4pt}
  Function $F$ calls $\createF(G)$:\vspace{-1ex} 
  \begin{codebox*}
     \zi \RComment $u$ is the strand in $F$ immediately before the \createF
     \zi \RComment $w$ is the strand in $F$ immediately after the \createF 
     \zi \RComment $v$ is the first strand of $G$
     \li $S_G \gets \MakeSet(\dssp, w)$ \lilabel{dsspcreate}
     \li $\proc{Attachify}(u)$   \lilabel{AttachifyCreate1}
     \li $A_v \gets \MakeSet(\dsnsp, v)$ and make $A_v$ attached. \lilabel{AttachifyCreate2}
     \li Add an arc from $\find{\dsnsp, u}$ to $A_v$ in $\cal R$. \lilabel{arcCreatorFut}
     \li $A_w \gets \MakeSet(\dsnsp, w)$ and make $A_w$ attached.  \lilabel{AttachifyCreate3}
     \li Add an arc from $\find{\dsnsp, u}$ to $A_w$ in $\cal R$ \lilabel{arcCreatorCont}
  \end{codebox*}
  \vspace{-.5ex}
\noindent\rule{\linewidth}{0.4pt}
  Function $G$ returns:\vspace{-1ex}
  % to function $F$ from a spawn or a \createF call:\vspace{-1ex}
  % \anote{I comment out the above because it's confusing ... this is
  % basically for a function returning, regardless G is spawned or a future, right?}  
  \begin{codebox*}
     \li $P_G \gets S_G$; deallocate $S_G$ \lilabel{dsspreturn}
  \end{codebox*}
  \vspace{-2ex}
\noindent\rule{\linewidth}{0.4pt}
  Function $F$ calls \getF($G$):\vspace{-1ex}
  \begin{codebox*}
%     \zi \RComment $u$ is the strand in $F$ immediately before the get 
%     \zi \RComment $v$ is the strand immediately after; $w$ is the last strand of $G$.  
%     \anote{I updated the comment above; check ...}
%     \anote{I also commented out \lilabel that doesn't seem to be used}
     \zi \RComment $u$ is the strand in $F$ that ended with the get 
     \zi \RComment $v$ is the strand immediately after $u$ in $F$ 
     \zi \RComment $w$ is the last strand of $G$.  
     \li $\proc{Attachify}(u)$  \lilabel{AttachifyGet1}
     \li $A_v \gets \MakeSet(\dsnsp, v)$ and make $A_v$ attached. \lilabel{AttachifyGet2}
     \li Add an arc from $\find{\dsnsp, u}$ to $A_v$ in $\cal R$  \lilabel{arcContGetter}
     \li Add an arc from $\find{\dsnsp, w}$ to $A_v$ in $\cal R$; 
     \zi \RComment $\find{\dsnsp, w}$ is guaranteed to be attached. %\lilabel{arcFutGetter}
  \end{codebox*}
  \end{minipage}%
  & 
  \begin{minipage}[t]{0.51\linewidth}
  \vspace{-2ex}
  \begin{codebox*}
    \Procname{$\proc{Attachify}(u)$ 
        \Comment{make the set containing $u$ attached if not already.}}
    \li $U_u \gets \proc{Find}(\dsnsp, u)$
    \li \If $U_u$ is unattached
    \li \Then mark $U_u$ as attached
    \li       add $U_u$ to $\cal R$
    \li       add the arc $(\attpred{U_u},U_u)$ to $\cal R$
        \End
  \end{codebox*}
  \vspace{-.5ex}
\noindent\rule{\linewidth}{0.4pt}
  Function $F$ calls \sync with child function $G$:\vspace{-1ex}
  \begin{codebox*}
    \li $S_F \gets S_F \cup P_G$; deallocate $P_G$ \lilabel{syncBegin}
    \li look at the corresponding fork
    \li let $f$ be the strand immediately preceding the fork
    \li let $s_1$ and $s_2$ be $f$'s two immediate successors of $f$
    \zi \RComment i.e., the first strand of $G$ and the first strand of 
                  the continuation
    \li let $j$ be the strand immediately after the sync
    \li let $t_1$ and $t_2$ be $j$'s immediate predecessors of the sync
    \zi \RComment i.e., the last strand of the $G$ and the continuation
    \li \If neither $\find{\dsnsp, t_1}$ nor $\find{\dsnsp, t_2}$ is attached
    \zi \RComment{No non-SP edges} \lilabel{unattachedUnionStart}
    \li \Then $\proc{Union}(\dsnsp, f,t_1)$ 
    \li    $\proc{Union}(\dsnsp, f,t_2)$
    \li    $\proc{Union}(\dsnsp, f,\MakeSet(j))$ \lilabel{unattachedUnionEnd}
    \li \ElseIf both $\find{\dsnsp, t_1}$ and $\find{\dsnsp, t_2}$ are attached \lilabel{twoAttachedSync}
    \li \Then $\proc{Attachify}(f)$ \lilabel{spawnAttachify}
    \li    add arc $(\find{\dsnsp, f},\find{\dsnsp, s_1})$ to $\cal R$ \lilabel{arcSourceChildren1}
    \li    add arc $(\find{\dsnsp, f},\find{\dsnsp, s_2})$ to $\cal R$ \lilabel{arcSourceChildren2}
    \li    $A_j = \MakeSet(\dsnsp, j)$ and make $A_j$ attached \lilabel{joinAttachify}
    \li    add a node $A_j$ to $\cal R$
% \anote{I split the following add arc to R into two statements
    \li    add arc $(\find{\dsnsp, t_1},A_j)$ to $\cal R$ \lilabel{arcChildrenSink1}
    \li    add arc $(\find{\dsnsp, t_2},A_j)$ to $\cal R$ \lilabel{arcChildrenSink2}
    \li \Else let $t_a$ be the attached one and $t_u$ be the \lilabel{oneAttachedSync}
                unattached one
    \li   correspondingly $s_a$ is attached and $s_u$ is unattached
    \li   \If $\find{\dsnsp, f}$ is not attached 
    \li   \Then $\proc{Union}(\dsnsp, s_a,f)$ \lilabel{singleUnionSrc}
          \End
    \li   $\proc{Union}(\dsnsp, t_a, \proc{Make-Set}(j))$ \lilabel{singleUnionSync}
    \li         $\attsucc{\find{\dsnsp, t_u}} \gets \find{\dsnsp, j}$ \lilabel{setAttSucc}
        \End
  \end{codebox*}
  \end{minipage}%
  \\ \hline
  \end{tabular}
\caption{The actions taken by the algorithm to maintain $\dssp$, $\dsnsp$ and $\cal R$}
\label{code:maintainReach}
\end{figure}

